Tag that issue: Applying API-domain labels in issue tracking systems

Labeling issues with the skills required to complete them can help contributors to choose tasks in Open Source Software projects. However, manually labeling issues is time-consuming and error-prone, and current automated approaches are mostly limited to classifying issues as bugs/non-bugs. We investigate the feasibility and relevance of automatically labeling issues with what we call "API-domains," which are high-level categories of APIs. Therefore, we posit that the APIs used in the source code affected by an issue can be a proxy for the type of skills (e.g., DB, security, UI) needed to work on the issue. We ran a user study (n=74) to assess API-domain labels' relevancy to potential contributors, leveraged the issues' descriptions and the project history to build prediction models, and validated the predictions with contributors (n=20) of the projects. Our results show that (i) newcomers to the project consider API-domain labels useful in choosing tasks, (ii) labels can be predicted with a precision of 84% and a recall of 78.6% on average, (iii) the results of the predictions reached up to 71.3% in precision and 52.5% in recall when training with a project and testing in another (transfer learning), and (iv) project contributors consider most of the predictions helpful in identifying needed skills. These findings suggest our approach can be applied in practice to automatically label issues, assisting developers in finding tasks that better match their skills.

==> sql.tex <==
% select distinct f.file_name from "API_specific" ap, "API" a, "file_API" fa, file f where ap.expert like 'Logging' and ap.api_name_fk = a.api_name and a.api_name = fa.api_name and fa.file_name = f.full_name and f.project = 'audacity' 

% audacity logging = 12 
% powertoys logging = 1
% rmca logging = 692
% cronos logging = 0
% jabref50 logging = 198

% audacity test = 0 
% powertoys test = 1
% rmca test = 4218
% cronos test = 0
% jabref50 test = 361

% audacity Internationalization = 0 
% powertoys Internationalization = 1
% rmca Internationalization = 58
% cronos Internationalization = 0
% jabref50 i18n = 14

% audacity security = 0 
% powertoys security = 0
% rmca security = 33
% cronos security = 7
% jabref50 security = 7

% audacity multimedia = 182 
% powertoys multimedia = 0
% rmca multimedia = 0
% cronos multimedia = 0
% jabref50 multimedia = 0

% audacity Computer Graphics = 5 
% powertoys Computer Graphics = 0
% rmca Computer Graphics = 0
% cronos Computer Graphics = 0
% jabref50 CG = 0

% SELECT java, COUNT(DISTINCT expert) AS numRows FROM apriori where java in  (select java from apriori where project = 'jabref50' and expert = 'i18n') group by java

% (select java from apriori where project = 'rmca' and expert = 'Logging')
%intersect
%(select java from apriori where project = 'rmca' and expert = 'Test')

% SELECT java 
%FROM apriori where project = 'jabref50' and expert = 'Test'

==> tables/CM-CronosH10.tex <==
% Cronos is in portuguese and therefore does not participate in the transfer learning experiment

==> tables/ITS.tex <==
\begin{landscape}
\begin{table}[]
\centering
\caption{Projects Mined and Issue Tracker Systems}
 \label{tab:projectsmined}

\begin{tabular}{l|l|l|l|l|c|c|c|c|c}
\hline
\textbf{Project} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Prog\\ Lang\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Issue\\ Tracker\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Extraction\\ Method\end{tabular}} &
  %\textbf{\begin{tabular}[c]{@{}l@{}}Linked\\ Data\end{tabular}} &
  %\textbf{\begin{tabular}[c]{@{}l@{}}Data\\ Source\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Vocab-\\ ulary\end{tabular}} &   \textbf{\begin{tabular}[c]{@{}l@{}}Issues \end{tabular}} &  
  \textbf{\begin{tabular}[c]{@{}l@{}}Pull\\ Requests\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Linked \\ Issues/PR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Source \\ files\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Distinct \\ APIs\end{tabular}} \\ \hline
JabRef &
  Java &
  GitHub &
  GitHub API V3 &
  %\begin{tabular}[c]{@{}l@{}}issues\\ pull requests\end{tabular} &
  %\begin{tabular}[c]{@{}l@{}}title,body \\ and comments\end{tabular} &
  EN & 4,471  & 1,966 & 1914 & 1,690  & 1,944\\
Audacity &
  C++ &
  GitHub &
  GitHub API V3 &
  %\begin{tabular}[c]{@{}l@{}}issues\\ pull requests\end{tabular} &
  %\begin{tabular}[c]{@{}l@{}}title,body \\ and comments\end{tabular} &
  EN &   1,440 & 310 & 341 & 624 & 1,478\\
PowerToys &
  C\# &
  GitHub &
  GitHub API V3 &
  %\begin{tabular}[c]{@{}l@{}}issues\\ pull requests\end{tabular} &
  %\begin{tabular}[c]{@{}l@{}}title,body \\ and comments\end{tabular} &
  EN & 12,571 & 853 & 1011 & 794 & 264 \\
RTTS &
  Java &
  Gerrit &
  Export CSV &
  %\begin{tabular}[c]{@{}l@{}}trouble id\\ change id\end{tabular} &
  %title, description &
  EN &  2,836 & 470 & 470 & 9,779 & 8,645\\
Cronos &
  Java &
  Jira/MTT &
  \begin{tabular}[c]{@{}l@{}}Export CSV/\\ TXT\end{tabular} &
  %\begin{tabular}[c]{@{}l@{}}key\\ revision\end{tabular} &
  %\begin{tabular}[c]{@{}l@{}}summary\\ description\end{tabular} &
  PT & 913 & 1075 & 206 & 220 & 441  \\
 \hline
 Total &&&&& 22,231 &	4,674	& 3942 & 13,107 &	12,772 \\
 \hline
\end{tabular}

\end{table}
\end{landscape}
%JabRef   & 4,471  & 1,966 & 1914 & 1,690  & 1,944    \\
%RxJava   & 6,765  & 1,938 & 1,870  & 416     \\
%Guava    & 3,590  & 263  & 3,011  & 1,676    \\
%Mockito  EN & 2,084  & 491  & 949   & 1,082    \\
%Presto   & 15,157 & 686  & 7,062  & 11,332   \\
%Total   & 32,067 & 5,344 & 14,582 & 16,450  
%Audacity &   1,440 & 310 & 341 & 624 & 1,478 \\
%PowerToys &  12,571 & 853 & 1011 & 794 & 264 \\
%Rmca &  2,836 & 470 & 470 & 9,779 & 8,645 \\
%Cronos &  913 & 1075 & 206 & 220 & 441 \\

%Total  & 49,827&	8,052	&25,999&	27,278  \\
%Total & 22,231 &	4,674	& 3942 & 13,107 &	12,772 

==> tables/ITS2.tex <==
\begin{table}[tb]
\centering
\scriptsize
\caption{Projects Mined and Issue Tracker Systems}
 \label{tab:projectsmined2}

\begin{tabular}{l|l|l|l|l|c|c|c|c|c}
\hline
\textbf{Project} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Prog\\ Lang\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Issue\\ Tracker\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Extraction\\ Method\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Vocab-\\ ulary\end{tabular}} & \textbf{Issues} & \textbf{\begin{tabular}[c]{@{}c@{}}Pull\\ Requests\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Linked\\ Issues/PR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Source\\ files\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Distinct\\ APIs\end{tabular}} \\ \hline
JabRef           & \multicolumn{1}{l|}{Java}                                                         & \multicolumn{1}{l|}{GitHub}                                                           & \multicolumn{1}{l|}{GitHub API V3}                                                        & EN                                                              & 4,471           & 1,966                                                            & 1914                                                                & 1,690                                                           & 1,944                                                            \\
Audacity         & \multicolumn{1}{l|}{C++}                                                          & \multicolumn{1}{l|}{GitHub}                                                           & \multicolumn{1}{l|}{GitHub API V3}                                                        & EN                                                              & 1,440           & 310                                                              & 341                                                                 & 624                                                             & 1,478                                                            \\
PowerToys        & \multicolumn{1}{l|}{C\#}                                                          & \multicolumn{1}{l|}{GitHub}                                                           & \multicolumn{1}{l|}{GitHub API V3}                                                        & EN                                                              & 12,571          & 853                                                              & 1011                                                                & 794                                                             & 264                                                              \\
RTTS             & \multicolumn{1}{l|}{Java}                                                         & \multicolumn{1}{l|}{Gerrit}                                                           & \multicolumn{1}{l|}{Export CSV}                                                           & EN                                                              & 2,836           & 470                                                              & 470                                                                 & 9,779                                                           & 8,645                                                            \\
Cronos           & \multicolumn{1}{l|}{Java}                                                         & \multicolumn{1}{l|}{Jira/MTT}                                                         & \multicolumn{1}{l|}{Export CSV/TXT}                                                       & PT                                                              & 913             & 1075                                                             & 206                                                                 & 220                                                             & 441                                                              \\ \hline
Total            & \multicolumn{4}{l|}{}                                                                                                                                                                                                                                                                                                                   & 22,231          & 4,674                                                            & 3,942                                                                & 13,107                                                          & 12,772                                                           \\ \hline
\end{tabular}
\end{table}

==> tables/ITSA.tex <==
\begin{table}[]
\centering
\caption{Projects Mined and Issue Tracker Systems}
 \label{tab:projectsminedA}
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Project} & \textbf{\begin{tabular}[c]{@{}l@{}}Prog\\ Lang\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Issue\\ Tracker\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Extraction\\ Method\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Vocab-\\ ulary\end{tabular}} \\ \hline
JabRef           & Java                                                         & GitHub                                                           & GitHub API V3                                                        & EN                                                              \\
Audacity         & C++                                                          & GitHub                                                           & GitHub API V3                                                        & EN                                                              \\
PowerToys        & C\#                                                          & GitHub                                                           & GitHub API V3                                                        & EN                                                              \\
RTTS             & Java                                                         & Gerrit                                                           & Export CSV                                                           & EN                                                              \\
Cronos           & Java                                                         & Jira/MTT                                                         & Export CSV/TXT                                                       & PT                                                              \\ \hline
\end{tabular}
\end{table}

==> tables/ITSB.tex <==
\begin{table}[]
\centering
\caption{Projects Mined Demographics}
 \label{tab:projectsminedB}
\begin{tabular}{l|c|c|c|c|c}
\hline
\textbf{Project} & \textbf{Issues} & \textbf{\begin{tabular}[c]{@{}c@{}}Pull\\ Requests\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Linked\\ Issues/PR\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Source\\ files\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Distinct\\ APIs\end{tabular}} \\ \hline
JabRef           & 4,471           & 1,966                                                            & 1914                                                                & 1,690                                                           & 1,944                                                            \\
Audacity         & 1,440           & 310                                                              & 341                                                                 & 624                                                             & 1,478                                                            \\
PowerToys        & 12,571          & 853                                                              & 1011                                                                & 794                                                             & 264                                                              \\
RTTS             & 2,836           & 470                                                              & 470                                                                 & 9,779                                                           & 8,645                                                            \\
Cronos           & 913             & 1075                                                             & 206                                                                 & 220                                                             & 441                                                              \\ \hline
Total            & 22,231          & 4,674                                                            & 3942                                                                & 13,107                                                          & 12,772                                                           \\ \hline
\end{tabular}
\end{table}

==> tables/demoWithTreatment.tex <==
\noindent\textbf{Comparison between API Labels and component}
Practitioners select marginally less API labels than students (66.8\% x 68.5\%). And practitioners select marginally more components labels than students (33.2\% x 31.5\%).

The same occurred when we compared the experienced and novice coders: more API labels preference from experienced coders (66.3\% x 68.1\%). And marginally more component labels from experienced coders (33.7\% x 31.9\%).

API labels were \textbf{more} selected than component with similar results from the industry (66.8\% x 33.2\%) and experienced (66.3\% x 33.7\%). The student (68.5\% x 31.5\%) demographic subgroup and the novice (68.1\% x 31.9\%) coders subgroup also had similar selections for the component labels.

\noindent\textbf{Comparison between API Labels and issue type}
Practitioners also selected more API labels (54.8\% x 52.1\%) than students and less issue type labels (45.2\% x 47.8\%) as well. And experienced coders selected more API labels than novice (60.4\% x 50.8\%) and less issue type than novice coders (39.6\% x 49.2\%).

API labels were \textbf{more} selected than issue type with a difference between industry (54.8\% x 45.2\%) and experienced (66.3\% x 33.7\%). The student (52.1\% x 47.8\%) demographic and the novice (50.8\% x 49.2\%) coders subgroup had similar selections for the issue type.

It suggests the API labels are perceived with more relevant a great difference from all subgroups than the component labels.  API labels also were perceived more relevance than the issue types with a marginal difference in the subgroups, except in the experienced coders where we could observe a greater difference.
\input{tables/APIxCompxTypeTreatment}

Table \ref{tab:resultsRQ2Dif} shows that p-values for all demographics are over the significance threshold ($>$0.05). 

The null hypothesis, states there is no significant difference between the expected and observed result, and here it means the two groups have the same distribution. So, the proportion of practitioners group and the students comparing the API labels to component labels is not significant, and $chi^2$=0.02, p=0.87,  with a small effect size (Cramer's V = 0.009). Comparing API labels to issue types we also did not observed a difference in proportions with $chi^2$=0.14, p=0.70, with small effect size (Cramer's V =0.02). Comparing the experienced coders and novice, there is not a difference in proportions from the API labels to the issue types, ($chi^2$=0.02, p=0.86) with a small effect size (Cramer's V =0.-1), and there is no difference in proportions comparing the API labels and the component labels ($chi^2$=0.11, p=0.08).

\input{tables/APILabels}

\MyBox{\textbf{\emph{RQ2 Summary.}} Our findings suggest that Title and Labels have important information for selecting an issue to work. API labels regions also increased the perception of the label region's relevancy. Comparing the demographic subgroups industry and experienced coders selected more and with same distribution the API labels than the Component labels and isue types. \XXX}

\section{Discussion}

This section discuss our results and future work. 

\noindent\textbf{Are API labels relevant?} The Table \ref{tab:resultsRQ2Dif} indicates how each demographic subset perceived the API labels' relevancy. Comparing with the component labels and issues types, all subgroups selected more the API labels and it might suggest a preference for the API labels. Our first insight was that the API labels could help newcomers, and could be more selected by the subgroups with less experience by providing them with more information to make a decision, but the result might suggest a more embracing preference for the API labels including experienced coders and those who work in the industry. %It might indicate the more the developer is closer to the project's technical skills, %or to the technology in the scope of this survey, 
%the more important it is to have detailed information about the API to solve an issue. 
This study enriches the previous literature (\ref{sec:related}) by adding new contextual information for developers that are trying to onboard to a new project. On the other hand, new hypotheses may be investigated to explore in depth the type of technology fit for labeling in the appropriate granularity. Those topics can be explored in a future work. 

It is also important to better investigate what will be most effective for helping new contributors in onboarding. In fact, one participant (P3BC) mentioned that ``UX aspects are important to address when labeling, pointing to the problems created by a possible label overhead''. 

\section{Conclusion}

We found all demographic groups select more the generated labels suggesting the API labels' relevance, comparing with the component labels.



Finally ,treatment group select  API labels more than component labels with a statistical difference, confirming our claim above about their usefulness.

==> tables/desired_labels.tex <==
\begin{table}[htb]
\centering
\caption{Labels desired by participants to select the issue}
\label{tab:desired_labels}

\begin{tabular}{|c|c|}
\hline
Desired Labels     & Participants who mentioned              \\ \hline
Type &
  \begin{tabular}[c]{@{}c@{}}P7B0, P11B0, P12B0, P13B0, P7C0, P8B1, P8P1\\ P4C1, P5N1, P21I1\end{tabular} \\ \hline
Priority &
  \begin{tabular}[c]{@{}c@{}}P3B0, P11I0, P22I0, P9B1, P5P1, P10P1, P15I1\\ P16I1, P17I1, P3N1\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}programming \\ language\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}P10B0, P13I0, P3N0, P6B1, P7B1, P3P1, P11P1\\ P22I1, P23I1\end{tabular} \\ \hline
Difficulty level   & P14B0, P21B0, P14I0, P3C0, P10I1, P11I1 \\ \hline
Technology         & P6B0, P10B0, P13I0, P4B1, P9B1, P18B0   \\ \hline
API                & P7B0, P12B0, P13B0, P7P0, P9B1                \\ \hline
Architecture layer & P4B0, P13B0, P7B1, P3N1                 \\ \hline
Status             & P5B0, P10I1, P16I1                      \\ \hline
GitHub info        & P10P0, P22I0                            \\ \hline
Database           & P13I0                                   \\ \hline
Framework          & P9B1                                    \\ \hline
%Library            & P9B1     = API                               \\ \hline
\end{tabular}
\end{table}



==> tables/open-question-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{comment}
\begin{table*}[]
 \caption{Open-ended question 1: Why the information you selected was relevant?}
 \label{tab:open-ended-Q1}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
{\color[HTML]{000000} \textbf{5W2H Question}}                                                           & {\color[HTML]{000000} \textbf{Code}}                                                                 & {\color[HTML]{000000} \textbf{Definition}}                                                                                                                               & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}What region has \\ this information?\end{tabular}}} \\ \hline
{\color[HTML]{000000} What is the issue}                                                                & {\color[HTML]{000000} Information about the issue}                                                   & {\color[HTML]{000000} Information about the issue}                                                                                                                       & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Title, Tags, Body, Comments, \\ Code Snipped\end{tabular}}  \\ \hline
{\color[HTML]{000000} What is the issue}                                                                & {\color[HTML]{000000} Type of the issue}                                                             & {\color[HTML]{000000} Issue type/classification}                                                                                                                         & {\color[HTML]{000000} Tags}                                                                                  \\ \hline
{\color[HTML]{000000} What is the issue}                                                                & {\color[HTML]{000000} Scenario of the issue}                                                         & {\color[HTML]{000000} Scenario of the issue}                                                                                                                             & {\color[HTML]{000000} Linked Issue, Comments}                                                                \\ \hline
{\color[HTML]{000000} Where is the issue}                                                               & {\color[HTML]{000000} Localize the issue}                                                            & {\color[HTML]{000000} Where in code is the issue happening}                                                                                                              & {\color[HTML]{000000} Code Snippet}                                                                          \\ \hline
{\color[HTML]{000000} Where is the issue}                                                               & {\color[HTML]{000000} Connected areas}                                                               & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}What areas of the system are connected \\ to the one with the issue\end{tabular}}                                       & {\color[HTML]{000000} Linked Issue, Comments}                                                                \\ \hline
{\color[HTML]{000000} Where is the issue}                                                               & {\color[HTML]{000000} Start Point}                                                                   & {\color[HTML]{000000} Where to go to solve the issue}                                                                                                                    & {\color[HTML]{000000} Body, Comments, Code Snippet}                                                          \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Previous Attempts}                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Previous attempts followed by people \\ who tried to solve the issue\end{tabular}}                                      & {\color[HTML]{000000} Comments, Linked Issue}                                                                \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Steps to Reproduce}                                                            & {\color[HTML]{000000} How to reproduce the issue}                                                                                                                        & {\color[HTML]{000000} Body, Comments}                                                                        \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Steps to Debug}                                                                & {\color[HTML]{000000} How to debug the issue}                                                                                                                            & {\color[HTML]{000000} Comments}                                                                              \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Challenges faced}                                                              & {\color[HTML]{000000} What challenges people have faced to solve}                                                                                                        & {\color[HTML]{000000} N/A}                                                                                   \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Expected behaviour}                                                            & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}How would it be the system's correct or \\ expected behaviour (without the issue)\end{tabular}}                         & {\color[HTML]{000000} Title, Body, Comments}                                                                 \\ \hline
{\color[HTML]{000000} How to solve the issue}                                                           & {\color[HTML]{000000} Suggested solutions}                                                           & {\color[HTML]{000000} What solutions are being suggested by others}                                                                                                      & {\color[HTML]{000000} Comments}                                                                              \\ \hline
{\color[HTML]{000000} Why is that an issue}                                                             & {\color[HTML]{000000} Goal to solve the issue}                                                       & {\color[HTML]{000000} What the issue was created for}                                                                                                                    & {\color[HTML]{000000} N/A}                                                                                   \\ \hline
{\color[HTML]{000000} Why is that an issue}                                                             & {\color[HTML]{000000} Benefits of solving the issue}                                                 & {\color[HTML]{000000} What benefits for users will this issue bring}                                                                                                     & {\color[HTML]{000000} N/A}                                                                                   \\ \hline
{\color[HTML]{000000} Who will solve the issue}                                                         & {\color[HTML]{000000} Required skills}                                                               & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}What skills or expertise are needed for a person \\ to have in order to solve the issue\end{tabular}}                   & {\color[HTML]{000000} Title, Tags}                                                                           \\ \hline
{\color[HTML]{000000} Who will solve the issue}                                                         & {\color[HTML]{000000} Experience level}                                                              & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}What experience level is needed for a person to \\ have in order to solve the issue (newcomer, senior...)\end{tabular}} & {\color[HTML]{000000} Title, Body, Comments}                                                                 \\ \hline
{\color[HTML]{000000} Who will solve the issue}                                                         & {\color[HTML]{000000} Feeling Safe}                                                                  & {\color[HTML]{000000} Feel safe to select the issue to solve}                                                                                                            & {\color[HTML]{000000} Body, Comments}                                                                        \\ \hline
{\color[HTML]{000000} Who will solve the issue}                                                         & {\color[HTML]{000000} Easy to Work}                                                                  & {\color[HTML]{000000} Consider easy to work on the issue}                                                                                                                & {\color[HTML]{000000} Title}                                                                                 \\ \hline
{\color[HTML]{000000} Who will solve the issue}                                                         & {\color[HTML]{000000} Getting Attracted}                                                             & {\color[HTML]{000000} Get interested to choose and solve the issue}                                                                                                      & {\color[HTML]{000000} Title, Tags, Body, Comments, Status}                                                   \\ \hline
{\color[HTML]{000000} How big is the issue}                                                             & {\color[HTML]{000000} Required effort}                                                               & {\color[HTML]{000000} How much effort is needed to solve the issue}                                                                                                      & {\color[HTML]{000000} Title, Body}                                                                           \\ \hline
{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}When the issue was \\ or will be solved?\end{tabular}} & {\color[HTML]{000000} Status open or closed}                                                         & {\color[HTML]{000000} Tag indicating if the issue is open or closed}                                                                                                     & {\color[HTML]{000000} Tags, Status}                                                                          \\ \hline
{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}When the issue was \\ or will be solved?\end{tabular}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Description of an \\ ongoing solution\end{tabular}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}More information about the status if the issue \\ has an ongoing solution\end{tabular}}                                 & {\color[HTML]{000000} Comments}                                                                              \\ \hline
\end{tabular}
\end{table*}
\end{comment}


==> tables/open-question-1a.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[tb]
\centering
\addtolength{\tabcolsep}{-3pt}
\fontsize{8pt}{10pt}\selectfont
 \caption{Open-ended question 1: Why the information you selected was relevant?}
 \label{tab:open-ended-Q1a}


\begin{tabular}{|llll|}
\hline
\multicolumn{4}{|c|}{Open Question 1: Why the information you selected was relevant?} \\ \hline
\multicolumn{1}{|l|}{5W2H Question} &
  \multicolumn{1}{l|}{Code} &
  \multicolumn{1}{l|}{Definition} &
  \begin{tabular}[c]{@{}l@{}}What region has \\ this information?\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{What is the issue}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Information about \\ the issue\end{tabular}} &
  \multicolumn{1}{l|}{Information about the issue} &
  \begin{tabular}[c]{@{}l@{}}Title, Label, Body, \\ Comments, Code Snipped\end{tabular} \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Type of the issue} &
  \multicolumn{1}{l|}{Issue type/classification} &
  Tags \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Scenario of the issue} &
  \multicolumn{1}{l|}{Scenario of the issue} &
  Linked Issue, Comments \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{Where is the issue}} &
  \multicolumn{1}{l|}{Localize the issue} &
  \multicolumn{1}{l|}{Where in code is the issue happening} &
  Code Snippet \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Connected areas} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}What areas of the system are connected \\ to the one with the issue\end{tabular}} &
  Linked Issue, Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Start Point} &
  \multicolumn{1}{l|}{Where to go to solve the issue} &
  \begin{tabular}[c]{@{}l@{}}Body, Comments, \\ Code Snippet\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\multirow{6}{*}{How to solve the issue}} &
  \multicolumn{1}{l|}{Previous Attempts} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Previous attempts followed by people \\ who tried to solve the issue\end{tabular}} &
  Comments, Linked Issue \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Steps to Reproduce} &
  \multicolumn{1}{l|}{How to reproduce the issue} &
  Body, Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Steps to Debug} &
  \multicolumn{1}{l|}{How to debug the issue} &
  Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Challenges faced} &
  \multicolumn{1}{l|}{What challenges people have faced to solve} &
  N/A \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Expected behaviour} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}How would it be the system's correct or \\ expected behaviour (without the issue)\end{tabular}} &
  Title, Body, Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Suggested solutions} &
  \multicolumn{1}{l|}{What solutions are being suggested by others} &
  Comments \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Why is that an issue}} &
  \multicolumn{1}{l|}{Goal to solve the issue} &
  \multicolumn{1}{l|}{What the issue was created for} &
  N/A \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Benefits of solving \\ the issue\end{tabular}} &
  \multicolumn{1}{l|}{What benefits for users will this issue bring} &
  N/A \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Who will solve the issue}} &
  \multicolumn{1}{l|}{Required skills} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}What skills or expertise are needed for a \\ person to have in order to solve the issue\end{tabular}} &
  Title, Tags \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Experience level} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}What experience level is needed for a \\ person to have in order to \\ solve the issue (newcomer, senior...)\end{tabular}} &
  Title, Body, Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Feeling Safe} &
  \multicolumn{1}{l|}{Feel safe to select the issue to solve} &
  Body, Comments \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Easy to Work} &
  \multicolumn{1}{l|}{Consider easy to work on the issue} &
  Title \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{Getting Attracted} &
  \multicolumn{1}{l|}{Get interested to choose and solve the issue} &
  \begin{tabular}[c]{@{}l@{}}Title, Tags, Body, \\ Comments, Status\end{tabular} \\ \hline
\multicolumn{1}{|l|}{How big is the issue} &
  \multicolumn{1}{l|}{Required effort} &
  \multicolumn{1}{l|}{How much effort is needed to solve the issue} &
  Title, Body \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}When the issue was \\ or will be solved?\end{tabular}}} &
  \multicolumn{1}{l|}{Status open or closed} &
  \multicolumn{1}{l|}{Tag indicating if the issue is open or closed} &
  Tags, Status \\ \cline{2-4} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Description of an \\ ongoing solution\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}More information about the status \\ if the issue has an ongoing solution\end{tabular}} &
  Comments \\ \hline
\end{tabular}


\end{table*}

==> tables/open-question-1b.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[tb]
\centering
\addtolength{\tabcolsep}{-3pt}
\fontsize{8pt}{10pt}\selectfont
 \caption{Open-ended question 1: Why the information you selected was relevant?}
 \label{tab:open-question-1b}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{tabular}{l|l|l|l}
\textbf{5W2H Question}                                                                             & \textbf{Code}                      & \textbf{Definition}                                                                                                                                  & \textbf{\begin{tabular}[c]{@{}l@{}}What region has \\ this information?\end{tabular}} \\ \hline
                                                                                                   & Information about the issue        & Information about the issue                                                                                                  & \begin{tabular}[c]{@{}l@{}}Title, Tags, Body, \\ Comments, Code Snipped\end{tabular}  \\
                                                                                                   & Type of the issue                  & Issue type/classification                                                                                                                            & Tags                                                                                  \\
\multirow{-3}{*}{What is the issue}                                                                & Scenario of the issue              & Scenario of the issue                                                                                                                                & Linked Issue, Comments                                                                \\ \hline
                                                                                                   & Localize the issue                 & Where in code is the issue happening                                                                                                                 & Code Snippet                                                                          \\
                                                                                                   & Connected areas                    & \begin{tabular}[c]{@{}l@{}}What areas of the system are connected \\ to the one with the issue\end{tabular}                                          & Linked Issue, Comments                                                                \\
\multirow{-3}{*}{Where is the issue}                                                               & Start Point                        & Where to go to solve the issue                                                                                                                       & Body, Comments, Code Snippet                                                          \\ \hline
                                                                                                   & Previous Attempts                  & \begin{tabular}[c]{@{}l@{}}Previous attempts followed by people \\ who tried to solve the issue\end{tabular}                                         & Comments, Linked Issue                                                                \\
                                                                                                   & Steps to Reproduce                 & How to reproduce the issue                                                                                                                           & Body, Comments                                                                        \\
                                                                                                   & Steps to Debug                     & How to debug the issue                                                                                                                               & Comments                                                                              \\
                                                                                                   & Challenges faced                   & What challenges people have faced to solve                                                                                                           & N/A                                                                                   \\
                                                                                                   & Expected behaviour                 & \begin{tabular}[c]{@{}l@{}}How would it be the system's correct \\ or expected behaviour (without the issue)\end{tabular}                            & Title, Body, Comments                                                                 \\
\multirow{-6}{*}{How to solve the issue}                                                           & Suggested solutions                & What solutions are being suggested by others                                                                                                         & Comments                                                                              \\ \hline
                                                                                                   & Goal to solve the issue            & What the issue was created for                                                                                                                       & N/A                                                                                   \\
\multirow{-2}{*}{Why is that an issue}                                                             & Benefits of solving the issue      & What benefits for users will this issue bring                                                                                                        & N/A                                                                                   \\ \hline
                                                                                                   & Required skills                    & \begin{tabular}[c]{@{}l@{}}What skills or expertise are needed for a \\ person to have in order to solve the issue\end{tabular}                      & Title, Tags                                                                           \\
                                                                                                   & Experience level                   & \begin{tabular}[c]{@{}l@{}}What experience level is needed for a \\ person to have in order to solve \\ the issue (newcomer, senior...)\end{tabular} & Title, Body, Comments                                                                 \\
                                                                                                   & Feeling Safe                       & Feel safe to select the issue to solve                                                                                                               & Body, Comments                                                                        \\
                                                                                                   & Easy to Work                       & Consider easy to work on the issue                                                                                                                   & Title                                                                                 \\
\multirow{-5}{*}{Who will solve the issue}                                                         & Getting Attracted                  & Get interested to choose and solve the issue                                                                                                         & \begin{tabular}[c]{@{}l@{}}Title, Tags, Body, \\ Comments, Status\end{tabular}        \\ \hline
How big is the issue                                                                               & Required effort                    & How much effort is needed to solve the issue                                                                                                         & Title, Body                                                                           \\ \hline
                                                                                                   & Status open or closed              & Tag indicating if the issue is open or closed                                                                                                        & Tags, Status                                                                          \\
\multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}When the issue was \\ or will be solved?\end{tabular}} & Description of an ongoing solution & \begin{tabular}[c]{@{}l@{}}More information about the status if the \\ issue has an ongoing solution\end{tabular}                                    & Comments                                                                             
\end{tabular}


\end{table*}

==> tables/open-question-2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
 \caption{Open-ended question 2: What kind of label would you like to see in the issues?}
 \label{tab:open-ended-Q2}

\begin{tabular}{|l|l|l|}
\hline
\textbf{Code}                            & \textbf{Definition}                                                                                                                                                                                                                                                      & \textbf{Examples}                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
Type                                     & \cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}The type of the issue, and possible types were suggested by \\ participants as bug, new feature, performance, enhancement, security\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}"A label that informs precisely which type of issue is." (P21I1)\\ "i will usually look for type:bug" (P7B0)\\ "type: performance, type: feature and type: enhancement" (P12B0)\\ "All issues should have a type so I can see if my skill set is useful." (P5N1)\end{tabular}                                                                                                      \\ \hline
Priority                                 & \begin{tabular}[c]{@{}l@{}}When the issue needs or should to be solved according to the impact \\ that having this issue to the business or client. Possible priorities suggested \\ by participants were major/minor, high, medium, low, critical, urgent.\end{tabular} & \begin{tabular}[c]{@{}l@{}}"One that indicates that the issue is critical/important" (P9B1)\\ "URGENT or similar tag" (P11I0)\\ "priority -\textgreater low, high, critical" (P17I1)\\ "business impact" (P10P1)\end{tabular}                                                                                                                                                                                 \\ \hline
Programming language                     & The programming language involved in (the solution of) the issue.                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}"I would have liked to see the programming language that the code was written in. \\ For example, if Java was primarily used to write the code, a "Code: Java" tag would \\ have been beneficial" (P3N0)\\ "Maybe an information about programming language" (P7B1)\\ "A label to specify the technology involved in the issue. \\ For example: java, nodejs" (P13I0)\end{tabular} \\ \hline
\cellcolor[HTML]{FFFFFF}Difficulty level & \begin{tabular}[c]{@{}l@{}}How hard is the issue to be solved. Possible levels suggested by participants\\  were good first issue, easy, medium, hard, good challenging issue\end{tabular}                                                                               & \begin{tabular}[c]{@{}l@{}}"Some "difficulty" indicator for the issue. Something like easy, medium, hard, \\ or colors to represent it." (P14B0)\\ "Besides the label "good first issue" it may be helpful create labels for \\ other level of issues." (P14I0)\\ Maybe "good challenging issue" (P3C0)\end{tabular}                                                                                          \\ \hline
Technology                               & \begin{tabular}[c]{@{}l@{}}Broader than programming language, framework, library, database. This is \\ about any technical detail or the technology involved on the issue\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}"Labels related to technologies involved" (P9B1)\\ "The technology used" (P4B1)\\ "Labels with technical information" (P18B0)\end{tabular}                                                                                                                                                                                                                                         \\ \hline
Architecture layer                       & \begin{tabular}[c]{@{}l@{}}The architecture layer of the software involved in the issue. Possible layers \\ suggested by participants were frontend, backend, interface.\end{tabular}                                                                                    & \begin{tabular}[c]{@{}l@{}}"Maybe an information if it is related to frontend, backend" (P7B1)\\ "Front-end, Interface" (P13B0)\\ "Frontend and Backend" (P4B0)\end{tabular}                                                                                                                                                                                                                                  \\ \hline
API                                      & The API involved in the issue (e.g. UI)                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}"i will usually look without API: User Interface." (P7B0)\\ "API: User Interface" (P12B0)\end{tabular}                                                                                                                                                                                                                                                                             \\ \hline
Status                                   & If the issue is open, closed or some solution is in progress                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}"A label showing if the issue has a fix or not" (P5B0)\\ "If it was successfully completed, if it is open" (P16I1)\end{tabular}                                                                                                                                                                                                                                                    \\ \hline
GitHub info                              & \begin{tabular}[c]{@{}l@{}}The branches and number of comments of the issue that can be \\ retrieved from GitHub\end{tabular}                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}"ranking about the most commented" (P10P0)\\ "branches" (P22I0)\end{tabular}                                                                                                                                                                                                                                                                                                       \\ \hline
Database                                 & \begin{tabular}[c]{@{}l@{}}More specific than technology, this is about the database involved \\ in (the solution of) the issue.\end{tabular}                                                                                                                            & \begin{tabular}[c]{@{}l@{}}"A label to specify the technology involved in the issue. \\ For example: postgrees" (P13I10)\end{tabular}                                                                                                                                                                                                                                                                         \\ \hline
\cellcolor[HTML]{FFFFFF}Framework        & \begin{tabular}[c]{@{}l@{}}More specific than programming language, this is about the framework \\ involved in (the solution of) the issue.\end{tabular}                                                                                                                 &                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{1-2}
\cellcolor[HTML]{FFFFFF}Library          & What part of the code, specifically the library involved in (the solution of) the issue.                                                                                                                                                                                 & \multirow{-2}{*}{"labels related to frameworks/libs involved" (P9B1)}                                                                                                                                                                                                                                                                                                                                         \\ \hline
\end{tabular}
\end{table*}

==> tables/projects.tex <==
\begin{table}[]
 \caption{Project's data mined}
 \label{tab:projects}

\begin{tabular}{rrrrrrrr}
Project &   \begin{tabular}[c]{@{}l@{}}Issues \end{tabular} &  Pull Requests & \begin{tabular}[c]{@{}l@{}}Linked \\ Issues/PR\end{tabular} & \begin{tabular}[c]{@{}l@{}}Source \\ files\end{tabular} & \begin{tabular}[c]{@{}l@{}}Distinct \\ APIs\end{tabular}   \\
\hline
JabRef   & 4,471  & 1,966 & 1914 & 1,690  & 1,944    \\
%RxJava   & 6,765  & 1,938 & 1,870  & 416     \\
%Guava    & 3,590  & 263  & 3,011  & 1,676    \\
%Mockito  EN & 2,084  & 491  & 949   & 1,082    \\
%Presto   & 15,157 & 686  & 7,062  & 11,332   \\
%Total   & 32,067 & 5,344 & 14,582 & 16,450  
Audacity &   1,440 & 310 & 341 & 624 & 1,478 \\
PowerToys &  12,571 & 853 & 1011 & 794 & 264 \\
Rmca &  2,836 & 470 & 470 & 9,779 & 8,645 \\
Cronos &  913 & 1075 & 206 & 220 & 441 \\
\hline
%Total  & 49,827&	8,052	&25,999&	27,278  \\
Total & 22,231 &	4,674	& 3942 & 13,107 &	12,772 \\
\hline
% commits 
% select count(*) from "pr"
% audacity 310 - powertoys 853 - rmca 470
% select distinct api_name from "API"
% rmca 8645 - audacity 1478 - powertoys 264

%38,465 + (
%select count(*) from pr_issue
% old 38465 - Audacity 1440 - PowerToys 12571 - Rmca 2836 - Cronos 

%Linked issues/PR: get the size of the binaries. Cronos 206, Rmca 470,  PowerToys 1011, Jabref_50_2 1914, audacity 341


\end{tabular}
\end{table}

==> tables/reasons_regions.tex <==
\begin{table}[htb]
\centering
\caption{Reasons presented by participants to consider the region of information from the issue's page as relevant to decide about selecting the issue}
\label{tab:reasons_regions}
\begin{tabular}{|l|l|}
\hline
\textbf{Reasons}      & \textbf{Regions from the Issue's Page}                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Information \\ about the issue\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Title, Labels, Body, \\ Comments, Code Snipped\end{tabular} \\ \hline
Type of the issue     & Labels                                \\ \hline
Scenario of the issue & Linked Issue, Comments                \\ \hline
Localize the issue    & Code Snippet                          \\ \hline
Connected areas       & Linked Issue, Comments                \\ \hline
Start Point           & Body, Comments, Code Snippet          \\ \hline
Previous Attempts     & Comments, Linked Issue                \\ \hline
Steps to Reproduce    & Body, Comments                        \\ \hline
Steps to Debug        & Comments                              \\ \hline
Challenges faced      & Comments                              \\ \hline
Expected behaviour    & Title, Body, Comments                 \\ \hline
Suggested solutions   & Comments                              \\ \hline
Required skills       & Title, Labels                           \\ \hline
Experience level      & Title, Body, Comments                 \\ \hline
Feeling Safe          & Body, Comments                        \\ \hline
Easy to Work          & Title                                 \\ \hline
Getting Attracted     & Title, Labels, Body, Comments, Status \\ \hline
Required effort       & Title, Body                           \\ \hline
Status open or closed & Labels, Status                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Description of an\\ ongoing solution\end{tabular} & Comments                                                                               \\ \hline
\end{tabular}
\end{table}


==> tables/repos.tex <==
\begin{table}[]
 \caption{Repositories mined}
 \label{tab:repos}

\begin{tabular}{rrrr}
Project & \begin{tabular}[c]{@{}l@{}}Programming \\ Language\end{tabular} & Repository & Language      \\
\hline
JabRef  & Java & GitHub & EN \\
%RxJava  & Java & GitHub & EN \\
%Guava   & Java & GitHub & EN \\
%Mockito & Java & GitHub & EN \\
%Presto  & Java & GitHub & EN \\
Audacity & C++ & GitHub & EN  \\
PowerToys & C\# & GitHub & EN  \\
Rmca & Java & Gerrit & EN  \\
Cronos & Java & Jira/MTT & BR  \\
\hline
% commits 
% select count(*) from "pr"
% audacity 310 - powertoys 853 - rmca 470
% select distinct api_name from "API"
% rmca 8645 - audacity 1478 - powertoys 264
\end{tabular}
\end{table}

==> tables/rv2.tex <==
\begin{table}[]
\caption{Reviewer 2 Comments. }
 \label{tab:rv2}


\begin{tabular}{|l|l|}
\hline
\textbf{Comments }                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \textbf{Answers}                                                                                                                          \\ \hline
Intro                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}The term "API" has never been introduced in the paper. Therefore, before using this acronym, \\ authors should mention what API stands for.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & R2.1                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Although the introduction mentions that choosing an issue is challenging for new contributors \\ to the project, the introduction needs to be more explicit about why helping new contributors is \\ important. Moreover, sometimes the paper focuses on how API-domain labels would benefit new \\ contributors but other times, it focuses on the usefulness of API-domain labels for all developers. \\ I recommend making this point clear in the introduction. Who are the primary beneficiaries of \\ the API-domain label?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & R2.2                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}The intro does not explain why studying RQ2.1, RQ2.2, and RQ2.3 is important and how \\ answering these research questions would contribute to the paper's main goal.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & R2.3                                                                                                                            \\ \hline
METHOD                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}In RQ.1, the paper mentioned that the authors need to evaluate the manually curated labels. \\ However, the authors have not explained why they need to manually create a dataset with \\ API-labels. Furthermore, RQ1 shouldn't be the first RQ in the study since the authors need to\\  answer RQ2 first to answer RQ1. Indeed, in their previous study, the current RQ1 goes after the \\ current RQ2. What was the reason for this change? The authors should re-think the order of the \\ RQs so that the narrative flows.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & R2.4                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}There needs to be an explanation of why it is important to answer RQ2.2 and RQ2.3. Are \\ the authors expecting to help practitioners or researchers with these specific RQs? \\ The paper, as it is, is focused on the usefulness of API-domain labels rather than on how \\ the best technique to develop/automate the process.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & R2.5                                                                                                                            \\ \hline
RELEVANCE OF THE LABELS TO OUTSIDERS (RQ1)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}1. This is the first time that the authors use the word "outsiders". To keep the terminology \\ consistent and avoid misunderstandings, I would recommend using "new contributors" instead.\\ 2.      It needs to be clarified how the API-domain labels for the JabRef issues page were \\ selected. As I understood, the authors previously identified the labels in a manual analysis. \\ So at this point is unclear to know how these API-domain labels were created/chosen.\\ 3.      The paper mentioned that the authors reached out to graduate data science students \\ from a university in Brazil since they are potential contributors to the JabRef project. \\ Why reach out to Brazilian students and not students from Oregon or Northern Arizona \\ universities? Why are these potential students contributors and no other students? \\ This link needs to be clarified.\\ 4.      Figure 2 is blurry. Moreover, due to data privacy concerns, I recommend \\ anonymizing the name/username of the developers that appear in Figure 2.\\ 5.      What does GSoC mean?\\ 6.      What are the squares inside the boxes in Figure 5? If they represent the categories, \\ note that there are 22 squares, and on Page 12, the text mentioned that the analysis revealed 21 categories.\\ 7.      The section explaining the 5WH2 analysis should be improved. After reading it, \\ I thought the text didn't flow in some parts—also, the categories needed to be clarified.\\ 8.      What are examples of "GitHub info" labels?\end{tabular} & \begin{tabular}[c]{@{}l@{}}R2.6\\ \\ R2.7\\ \\ \\ R2.8\\ \\ \\ \\ \\ R2.9\\ \\ R2.10\\ R2.11\\ \\ R2.12\\ \\ R2.13\end{tabular} \\ \hline
LABEL PREDICTION (RQ2)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}1. To improve the readability of Table 5, split the Colum "Stars/Forks" into "stars" and "Forks". \\ Please, do the same with Closed PR, and Closed Issues\\ 2.      Previous studies have shown that some pull requests are merged without traces in the GitHub \\ UI and, therefore, without traces in the GitHub API. How have the authors mitigated this threat?\\ 3.      The authors restricted the data collection to 4 months (August to November 2022). I\\ s there any explanation for this?\\ 4.      Add the reference for the NLP Python package spacy\\ 5.      Experts were given a list with 32 "first tokens" and 73 "second tokens", \\ I missed how these numbers (32 and 73) were calculated.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & \begin{tabular}[c]{@{}l@{}}R2.14\\ \\ R2.15\\ \\ R2.16\\ \\ R2.17\\ \\ \\ R2.18\end{tabular}                                    \\ \hline
RQ3 EVALUATING THE API-DOMAIN LABELS WITH DEVELOPERS                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}The authors asked three questions to participants: (1) How important do they consider these labels, \\ (2) why, and (3) What labels are missing. While this section answered the first questions, there are \\ no answers for the second and third questions. Could the authors explain why?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & R2.19                                                                                                                           \\ \hline
Discussion                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}1.      In the results from RQ1, the authors found that participants from the industry selected \\ 1.9 times more API-domain labels than students. I would like to see more discussion about \\ this since students were potential new contributors to the project.\\ 2.      Also, it was interesting to see that experience coders selected more API than the novice. \\ This will need more discussion as the paper poses that using API-domain labels would benefit \\ newcomers (novice), and it seems that this is not the case.\\ 3.      In RQ2, the authors filtered out APIs not found in the latest version of the source code to \\ avoid recommending APIs in the source code that were no longer used in the project. If the \\ purpose of the paper is to propose this approach, it would be helpful to discuss how the authors \\ think this filtering can be automated.\\ 4.      The authors mentioned that the 5W2H analysis might help understand what should be \\ written in issues. And it proposes using templates in the future. However, there exist current \\ templates to write proper issues. The authors removed these templates for their NLP analysis. \\ So, I'm wondering how different the templates proposed by the authors would be compared \\ to the existing templates .How they would help newcomers.\end{tabular}                                                                                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}R2.20\\ \\ \\ R2.21\\ \\ \\ \\ R2.22\\ \\ \\ \\ \\ R2.23\end{tabular}                                \\ \hline
\end{tabular}
\end{table}

==> tables/rv3.tex <==
\begin{table}[]

\caption{Reviewer 3 Comments. }
 \label{tab:rv3}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{tabular}{|l|l|}
\hline
\textbf{Comments}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & \textbf{Answers}                                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}The assessment on learning transfer is shallow. It includes a small number of projects, \\ and authors themselves show how it may depend a lot on the specific characteristics of projects. \\ However, this could also be useful to transfer to other projects of similar characteristics.\\ * I couldn't find the reproduction package, the link provided seems to be wrong.\\ * There are some minor methodological details that could be described better, see other comments below.\\ Review criteria:\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}XXXX\\ \\ \\ R3.1\\ \\ XXXX\end{tabular}                         \\ \hline
* Soundness:                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &                                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}I find a minor issues in the first study, about the convenience of the API labels vs the labels \\ produced by the project: to which extent the study is measuring not the convenience of \\ having API labels, but how good or bad are labels produced by the project? Even when \\ I think this is not a major issue, I think it should be commented as a potential threat to validity.\\ \\ For this same study, another potential threat that (in my opinion) should be highlighted is to \\ which extent answers by subjects are good. Since they didn't actually try to fix the labels \\ (at least, as I understood, they didn't), maybe their judgment was not right, and they used \\ information (regions) that "seemed to them to be ok", but in fact, they were wrong, and the \\ information they used didn't help to select the most appropriate issues: they only would\\  know definitely if they actually tried to fix the issues. Again, I see this as a minor issue, \\ but I would mention it clearly as a potential threat to validity.\\ \\ In the case of the study on transfer learning, maybe it would be better to compare not the \\ training on all for projects for each of them, but of "the other three projects" for each of them. \\ If this is not the case, it would be interesting to explain why. If it is, and the study can be made, \\ maybe it would be more accurate to run it, and report its results instead of the ones currently reported.\end{tabular} & \begin{tabular}[c]{@{}l@{}}R3.2\\ \\ \\ \\ \\ R3.3\\ \\ \\ \\ \\ \\ \\ \\ R3.4\end{tabular} \\ \hline
* Significance:                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}The studies presented in the paper are clearly significant, both to researchers, since they provide \\ insight on how to automatically label issues with API-related tags, and to developers, since they \\ could benefit from this automatic tagging. In particular, since the results shown in the paper could \\ lead to reducing the effort needed for tagging issues automatically, and that they also show that \\ these tags could help to select more appropriate issues, the paper seems to me very significant.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & XXXX                                                                                        \\ \hline
* Novelty:                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}To my knowledge, the work presented in the paper is novel. Previous work is, in my opinion, \\ adequately cited, and used to put in context the research presented in the paper.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & XXXX                                                                                        \\ \hline
* Verifiability and transparency:                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &                                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Procedures and methods are described in general in good detail, although having access to the \\ scripts used for the analysis would be convenient to easy understanding and applicability.\\ \\ I've tried the URL https://zenodo.org/record/6869246.YvsJS-zML0o which is said to give \\ access to the data related to the paper. But I got "Page not found". Maybe there is a typo in \\ the link? To better assess on verifiability and transparency, it would be convenient to have access to this data.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}XXXX\\ \\ \\ R3.1\end{tabular}                                   \\ \hline
* Presentation:                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}The presentation is good. The paper is in general easy to read and understand, and includes \\ enough detail to follow all the methods and procedures. Some more detailed comments on \\ specific parts of the paper are mentioned below, under "other comments".\\ \\ In the specific case of captions for figures, and some tables, it would be convenient to make \\ them more descriptive. Most of them are too terse, and it is difficult to understand their meaning, \\ in some cases even after reading the text referencing them.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}XXXX\\ \\ \\ \\ R3.5\end{tabular}                                \\ \hline
\end{tabular}
\end{table}

==> tables/rv3M.tex <==
\begin{table}[]
\caption{Reviewer 3 Other Comments. }
 \label{tab:rv3M}


\begin{tabular}{|l|l|}
\hline
\textbf{Other comments}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \textbf{Answers} \\ \hline
Abstract: "can help contributors choose tasks" -\textgreater{}(?) "can help contributors to choose tasks"                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & R3.M1   \\ \hline
\begin{tabular}[c]{@{}l@{}}Abstract: "as a bug/non-bug" -\textgreater "as bug/non-bug" or maybe "as a bugs/non-bugs" (having into \\ account that we're talking about "bugs", in plural.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & R3.M2   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 5: RQ 2.2: "using data from all projects" Wouldn't it be more exact to say "from other projects"? \\ Because even when data from all projects in the study is used, in fact the question which is addressed \\ is if data from other projects can be used to label the project of interest.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & R3.M3   \\ \hline
Page 5: "free code": I'm not sure what does this refer to.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & R3.M4   \\ \hline
Page 7, Fig 1, caption: "research method" -\textgreater Maybe "research methods" would be better.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & R3.M6   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 9: "We used a preliminary version of our prediction model to generate the issues." -\textgreater \\ Maybe "labels" instead of "issues"??\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & R3.M7   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 10, Fig 2: Consider using the actual text of an exemplary issue instead of the lorem \\ ipsum text. I think that would help to understand the different regions in the figure.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & R3.M5   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 14, Fig 4: Please, explain in the caption in more detail what is represented in the figures. \\ I know that there are more details in the text, but still, it would be convenient to have most or all \\ the information to understand the figures already in the caption. For instance, "density probability" \\ of what exactly? What does "API x Type" mean? And so on...\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & R3.M8   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 14: "To evaluate the information that should be used to build the classifiers to predict the\\  API-domain". However, the information that is captured, apparently, has more to do with how \\ subjects used information to decide if the task was appropriate to them, than to decide on the API-domain. \\ It would be convenient to explain why these two apparently different processes are related \\ (or why I'm wrong and I didn't understand the processes).\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                             & R3.6    \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 16: "critical/important" and "urgent" are usually in different dimensions,. \\ The first one talks about the importance of the bug report, the second one about their urgency. \\ Granted, both may be correlated in many cases, but one can easily think about bugs that are urgent \\ to fix, but not important, and the other way around. Some clarification on these would be convenient, \\ and also some explanation about why both categories are used to estimate (to some extent) urgency.\end{tabular}                                                                                                                                                                                                                                                                                                                                                              & R3.M9   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 18: "We also conducted experiments using another modern text classification\\ algorithm, BERT" Even when this paper is an extension of the previous paper in MSR, \\ I think that it would be better to frame the description of the method in section 5.1 as \\ "we use two methods, with two different classification algorithms", and then describe both of them. \\ And then (or previously), describe the projects used to test the methods. In other words, instead of \\ presenting the BERT method as a kind of a complement (which maybe was the case "historically"), \\ just present both methods and their results in equal terms (if convenient, mentioning the previous study). \\ This would help to better understand this paper if you didn't read the previous one. In fact, later sections, \\ such as 5.1.3, are already framed in this way.\end{tabular} & R3.7    \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 19: "MTT (Minds At Work Time Tracker)": Maybe the explanation \\ of the meaning of MTT would be better right after the first occurrence of MTT.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & R3.M10  \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 19, Table 6: Cronos is a project with the vocabulary of the issue tracking in \\ Brazilian Portuguese, if I understand well the table. But what about the names used in the \\ source code=? Are they also in BR or in EN? It would be convenient to clarify this somewhere \\ (not necessarily in the table), because it seems the methods used to classify code elements in \\ high-level APIs are for English only (if I understood well the discussion in pages 21, 22.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                      & R3.8    \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 23: "the uncleaned corpus increased the performance of BERT and the accuracy of \\ predictions": this is an assumption, or a fact that was checked? If so, how?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & R3.13   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 24: "We ran the classifiers using the Python sklearn package and tested several parameters." \\ I understand that this was the case for all classifiers except for BERT \\ (which is described in the next paragraph). If this is the case, please clarify.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & R3.M11  \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 26, Fig 7: If this figure is about all projects together (I think so, but I'm not completely sure), please specify.\\ \\ Page 27, Fig 8. Same.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & R3.5    \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 30: "Random Forest (RF) was the best model when compared to Decision Tree (DT)," \\ Even when results show this, maybe it would be convenient to explain also that differences \\ between some classifiers (eg RF and DT) are quite small, and maybe different projects, \\ results could be (somewhat) different.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & R3.9    \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 32: "Contributors assessment". I understand that each developer was shown \\ issues of their own project. If so, please clarify (if that is already detailed, and \\ I just misread it, please ignore this comment).\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             & R3.10   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 33: "A total of 13 contributors assessed the labels generated for 24 tasks." How many issues was presented \\ each developer? I mean, all 13 contributors were presented with 24 issues, or 24 issues were presented to one \\ of the 13 contributors? Besides, are you using "task" instead of "issue" now for some reason? If not,\\  I think it would be better to stick to "issue", to avoid confusion.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                      & R3.11   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 34: "What characteristics developer would like to see on labels?" -\textgreater \\ "What characteristics would a developer like to see on labels?"\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & R2.23   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 36, Fig 13: It would be convenient to provide some more detail in the caption, at least\\  explaining what the heatmap shows (what's the metric mapped to colors)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & R3.M14   \\ \hline
\begin{tabular}[c]{@{}l@{}}Page 38: "the BERT metrics got closer to the other classifiers". But maybe not much closer= It would be \\ interesting to include some quantification in the discussion. Even when it is likely that training BERT \\ with more issues could improve results, it is not clear that it would come close to the other classifiers, \\ which seem to have much better numbers.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & R3.12   \\ \hline
Page 43: "manually examined 100 tasks from the projects". Same comment as above about the word "task".                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & R3.M13   \\ \hline
Page 44: "domains, sizes, and languages,": I suggest "natural languages", to avoid confusion.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & R3.M12   \\ \hline
\end{tabular}
\end{table}

==> tables/survey_demo.tex <==
\begin{table}[htb]
\centering
\caption{Demographics Subsets for the Experiment's Participants}
\label{tab:demographics}

\begin{tabular}{lllllll}
\cline{1-3} \cline{5-7}
\multicolumn{1}{|l|}{Role}                                                               & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience with \\ JabRef technology\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Practitioner}                                                       & \multicolumn{1}{l|}{41} & \multicolumn{1}{l|}{55.5} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{High Experience}                                                              & \multicolumn{1}{l|}{31} & \multicolumn{1}{l|}{42}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Student}                                                            & \multicolumn{1}{l|}{33} & \multicolumn{1}{l|}{44.5} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Low Experience}                                                               & \multicolumn{1}{l|}{43} & \multicolumn{1}{l|}{58}   \\ \cline{1-3} \cline{5-7} 
                                                                                         &                         &                           &                       &                                                                                                 &                         &                           \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ Coder\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ OSS Contributor\end{tabular}}   & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Experienced}                                                        & \multicolumn{1}{l|}{28} & \multicolumn{1}{l|}{38}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Experienced}                                                                & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{13.5} \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Novice}                                                             & \multicolumn{1}{l|}{46} & \multicolumn{1}{l|}{62}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Novice}                                                                     & \multicolumn{1}{l|}{64} & \multicolumn{1}{l|}{86.5} \\ \cline{1-3} \cline{5-7} 
\end{tabular}
\end{table}

==> tables/survey_demoT.tex <==
\begin{table}[htb]
\centering
\caption{Demographics Subsets for the Experiment's Participants}
\label{tab:demographics}

\begin{tabular}{lllllll}
\cline{1-3} \cline{5-7}
\multicolumn{1}{|l|}{Role}                                                               & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience with \\ JabRef technology\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Practitioner}                                                       & \multicolumn{1}{l|}{23} & \multicolumn{1}{l|}{56.1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{High Experience}                                                              & \multicolumn{1}{l|}{17} & \multicolumn{1}{l|}{41.5}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Student}                                                            & \multicolumn{1}{l|}{18} & \multicolumn{1}{l|}{43.9} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Low Experience}                                                               & \multicolumn{1}{l|}{24} & \multicolumn{1}{l|}{58.5}   \\ \cline{1-3} \cline{5-7} 
                                                                                         &                         &                           &                       &                                                                                                 &                         &                           \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ Coder\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ OSS Contributor\end{tabular}}   & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Experienced}                                                        & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{26.8}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Experienced}                                                                & \multicolumn{1}{l|}{4} & \multicolumn{1}{l|}{9.8} \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Novice}                                                             & \multicolumn{1}{l|}{30} & \multicolumn{1}{l|}{73.2}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Novice}                                                                     & \multicolumn{1}{l|}{37} & \multicolumn{1}{l|}{90.2} \\ \cline{1-3} \cline{5-7} 
\end{tabular}
\end{table}
